Deep Learning Transient Detection with VERITAS

Ground-based $\gamma$-ray observatories, such as the VERITAS array of imaging atmospheric Cherenkov telescopes, provide insight into very-high-energy (VHE, $\mathrm{E}>100\,\mathrm{GeV}$) astrophysical transient events. Examples include the evaporation of primordial black holes, gamma-ray bursts and flaring blazars. Identifying such events with a serendipitous location and time of occurrence is difficult. Thus, employing a robust search method becomes crucial. An implementation of a transient detection method based on deep-learning techniques for VERITAS will be presented. This data-driven approach significantly reduces the dependency on the characterization of the instrument response and the modelling of the expected transient signal. The response of the instrument is affected by various factors, such as the elevation of the source and the night sky background. The study of these effects allows enhancing the deep learning method with additional parameters to infer their influences on the data. This improves the performance and stability for a wide range of observational conditions. We illustrate our method for an historic flare of the blazar BL Lac that was detected by VERITAS in October 2016. We find a promising performance for the detection of such a flare in timescales of minutes that compares well with the VERITAS standard analysis.

==> backup.tex <==
% more description of cuts. Probably not required and should be saved for thesis. Also would need to be improved!
\iffalse
Frequently, a short strong illumination of the camera can cause spikes or also drops in the L3 rate.
A spike search is applied, to remove these if they affect more than 2 seconds.
The moon-rise and -set can cause a change in the response in the time scales of several minutes that is reflected in a change of the L3 rate.
If only parts of the run are affected, a change of the L3 rate is expected within the rate.
We search for such events by testing, whether the L3 rate can be described by a linear curve or if a piece-wise linear function provides a better description.
Due to their large amount of variety, the automatic identification of clouds is challenging.
We make use of the fact that influences are expected as well in the L3 rate as in the FIR temperature.
The values are interpolated to obtain a sample value for both curves at each second to significant outliers in the L3-FIR.
Both values are normalized to the expected standard deviation for good observation.
The L3 rate is a stochastic process with an expected standard error of $\sigma_{\mathrm{L3}}=\sqrt{L3}$.
The typical deviation of the FIR temperature is defined as the $95\%$ quantile for clearly good runs. 
For each run, the normal value in the L3-FIR space is defined as the densest point that is obtained by a kernel density estimate.
Having the samples normalized to the expected fluctuations, we define outliers to be samples that are more than $3\sigma$ away from this central point.
To ensure, that only data that is really affected by the clouds is detected, we furthermore require a correlation of the FIR temperature and the L3 rate calculated using Spearman's rank correlation efficient.
If an outlier is detected while at the same time a correlation is found, we define set a time cut.

After the definition of these time cuts, we run a final validation on the surviving periods.
We discard periods that are shorter than 5 minutes and that have a slope in the L3 rate that is inconsistent with a constant.
The latter could either be caused by a change in the pointing elevation in the course of the run or by a change of the night sky background i.e. due to changes of the moon elevation.
We test for these influences by searching for correlations.
While the DL transient detection method should be able to deal with such slow changes of the response of the instrument, the investigation of these cases is beyond the scope of this work.
\fi
